Answer Set Solving with Bounded Treewidth Revisited

Parameterized algorithms are a way to solve hard problems more efficiently, given that a specific parameter of the input is small. In this paper, we apply this idea to the field of answer set programming (ASP). To this end, we propose two kinds of graph representations of programs to exploit their treewidth as a parameter. Treewidth roughly measures to which extent the internal structure of a program resembles a tree. Our main contribution is the design of parameterized dynamic programming algorithms, which run in linear time if the treewidth and weights of the given program are bounded. Compared to previous work, our algorithms handle the full syntax of ASP. Finally, we report on an empirical evaluation that shows good runtime behaviour for benchmark instances of low treewidth, especially for counting answer sets.

==> commands.tex <==
% Misc
\newcommand{\dneg}{\ensuremath{\operatorname{not}\,}}
\newcommand{\la}{\ensuremath{\leftarrow}}
\newcommand{\HU}[1]{\ensuremath{\mathcal{U}_#1}}
\newcommand{\HB}[1]{\ensuremath{\mathcal{B}_#1}}
\newcommand{\etal}{\emph{{et al}.}\@\xspace}
\newcommand{\eg}{e.g.,\@\xspace}
\newcommand{\ie}{i.e.,\@\xspace}
\newcommand{\wrt}{w.r.t.\@\xspace}
\newcommand{\dflat}{\mbox{D-FLAT}}
\renewcommand{\O}{\mathcal{O}}
\newcommand{\problem}[1]{\textsc{#1}}
\newcommand{\predicate}[1]{\texttt{\small #1}}
\newcommand{\dflatItem}[1]{\texttt{#1}}
\newcommand{\I}{\mathcal{I}}
\newcommand\pair[2]{\left< #1,#2 \right>}
\newcommand\tuple[1]{\left< #1 \right>}

\newcommand{\minSat}{\problem{$\subseteq$-Minimal Sat}}
\newcommand{\minDomSet}{\problem{$\subseteq$-Minimal Dominating Set}}
% todo
\newcommand{\todoi}[1]{\todo[inline]{#1}}

% complexity
\newcommand{\complexityclass}[1]{\ensuremath{\mathsf{#1}}}
\newcommand{\Sp}[1]{\complexityclass{\Sigma^P_{#1}}}
\newcommand{\Pp}[1]{\complexityclass{\Pi^P_{#1}}}
%\newcommand{\NP}{\complexityclass{NP}}
\newcommand{\coNP}{\complexityclass{\text{co-}NP}}
\newcommand{\DP}{\complexityclass{D^P}}
%\newcommand{\PSPACE}{\mbox{\rm PSPACE}}

% http://tex.stackexchange.com/questions/112204/how-to-vertically-center-the-vdots-in-this-node
\makeatletter
\DeclareRobustCommand{\rvdots}{%
  \vbox{
    \baselineskip4\p@\lineskiplimit\z@
    \kern-\p@
    \hbox{.}\hbox{.}\hbox{.}
  }}
\makeatother

% Algorithms
\newcommand{\eps}{\ensuremath{\operatorname{extensionPointers}}}
\newcommand{\cost}{\ensuremath{\operatorname{cost}}}
\newcommand{\type}{\ensuremath{\operatorname{type}}}
\newcommand{\solCount}{\ensuremath{\operatorname{count}}}


==> graph0/tables/join.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$\langle M_i \rangle$}\\
\hline\hline
%$1$ & & & \\\hline
%\multirow{1}{*}{$2$} & & \multirow{1}{*}{} & $1$ & &\\\hline
$\langle \emptyset \rangle$ \\\hline
$\langle \{a\} \rangle$\\
\end{tabular}


==> graph0/tables/join_asp.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$\langle M_i, C_j \rangle$}\\
\hline\hline
%$1$ & & & \\\hline
%\multirow{1}{*}{$2$} & & \multirow{1}{*}{} & $1$ & &\\\hline
$\langle \emptyset, \emptyset \rangle$\\\hline
$\langle \{a\}, \emptyset \rangle $\\\hline
$\langle \{a\}, \{\{a\}\} \rangle $\\
\end{tabular}


==> graph0/tables/join_aspnum.tex <==
\begin{tabular}{c}
\multirow{1}{*}{$i$}\\
\hline\hline
%$1$ & & & \\\hline
%\multirow{1}{*}{$2$} & & \multirow{1}{*}{} & $1$ & &\\\hline
$3.1$\\\hline
$3.2\text{a}$\\\hline
$3.2\text{b}$\\
\end{tabular}


==> graph0/tables/join_aspnumb.tex <==
\begin{tabular}{c}
\multirow{1}{*}{$j$}\\
\hline\hline
%$1$ & & & \\\hline
%\multirow{1}{*}{$2$} & & \multirow{1}{*}{} & $1$ & &\\\hline
\\\hline
\\\hline
$3.2\text{b}.1$\\
\end{tabular}


==> graph0/tables/joinnum.tex <==
\begin{tabular}{c}
\multirow{1}{*}{$i$}\\
\hline\hline
%$1$ & & & \\\hline
%\multirow{1}{*}{$2$} & & \multirow{1}{*}{} & $1$ & &\\\hline
$3.1$ \\\hline
$3.2$\\
\end{tabular}


==> graph0/tables/leaf0.tex <==
\begin{tabular}{l}
\multicolumn{1}{l}{$\langle M_i \rangle$}\\
%& $a$ & $b$ & $c$\\
\hline\hline
$\langle\{c\}\rangle$\\\hline
$\langle\{a\}\rangle$\\\hline
$\langle\{a,c\}\rangle$\\\hline
$\langle\{b,c\}\rangle$\\\hline
$\langle\{a,b,c\}\rangle$\\
\end{tabular}


==> graph0/tables/leaf0_asp.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$\langle M_i, C_j \rangle $}\\
\hline\hline
$\langle \{c\}, \emptyset \rangle $\\\hline
%$1.1$ & & & T\\\hline
$\langle \{a\}, \emptyset \rangle $\\\hline
%$1.2$ & T & &\\\hline
$\langle \{a,c\}, \{\{a\}\} \rangle $\\\hline
%$1.3$ & T & & T & $1.3.1$ & T&\\\hline
$\langle \{b,c\}, \emptyset \rangle $\\\hline
$\langle \{a,b,c\}, \{\{a\}\} \rangle $\\
%$1.4$ & & T & T\\\hline
%$1.5$ & T & T & T & $1.5.1$ & T&\\
\end{tabular}


==> graph0/tables/leaf0_aspnum.tex <==
\begin{tabular}{c}
\multirow{1}{*}{$i$}\\
\hline\hline
$1.1$\\\hline
$1.2$\\\hline
$1.3$\\\hline
$1.4$\\\hline
$1.5$
\end{tabular}



==> graph0/tables/leaf0_aspnumb.tex <==
\begin{tabular}{c}
\multirow{1}{*}{$j$}\\
\hline\hline
\\\hline
\\\hline
$1.3.1$\\\hline
\\\hline
$1.5.1$\\
\end{tabular}


==> graph0/tables/leaf0num.tex <==
\begin{tabular}{c}
\multirow{1}{*}{$i$}\\ % & \multicolumn{1}{c}{$M_i$}\\
%& $a$ & $b$ & $c$\\
\hline\hline
$1.1$ \\\hline
$1.2$ \\\hline
$1.3$ \\\hline
$1.4$ \\\hline
$1.5$ \\
\end{tabular}


==> graph0/tables/leaf1.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$\langle M_i \rangle$}\\ % & \multicolumn{2}{c}{$M_i$}\\
%& $a$ & $d$ \\
\hline\hline
$\langle \{a\}\rangle$\\\hline
$\langle \{d\}\rangle$\\\hline
$\langle \{a,d\}\rangle$\\
\end{tabular}


==> graph0/tables/leaf1_asp.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$\langle M_i, C_j \rangle $}\\
\hline\hline
$\langle \{ a\}, \emptyset \rangle$\\\hline
$\langle \{d\}, \emptyset \rangle $\\\hline
$\langle \{a,d\}, \{\{a\}, $\\
$\qquad\qquad \{d\}\}\rangle$\\
\end{tabular}


==> graph0/tables/leaf1_aspnum.tex <==
\begin{tabular}{c}
\multirow{1}{*}{$i$}\\
\hline\hline
$2.1$\\\hline
$2.2$\\\hline
\multirow{2}{*}{$2.3$}\\
\end{tabular}


==> graph0/tables/leaf1_aspnumb.tex <==
\begin{tabular}{c}
\multirow{1}{*}{$j$}\\
\hline\hline
\\\hline
\\\hline
$2.3.1$\\
$2.3.2$\\
\end{tabular}


==> graph0/tables/leaf1num.tex <==
\begin{tabular}{c}
\multirow{1}{*}{$i$}\\ % & \multicolumn{2}{c}{$M_i$}\\
%& $a$ & $d$ \\
\hline\hline
$2.1$\\\hline
$2.2$\\\hline
$2.3$\\
\end{tabular}


==> graph0/tables/tables.tex <==
\begin{tikzpicture}[node distance=1mm]
%\tikzset{every node/.style=tdnode}
\tikzset{every path/.style=thick}

%\node (leaf1) [stdnode,label={[tdlabel, xshift=-0.1cm]left:$\tab{t_1}$}]{\input{graph0/tables/leaf0}};
\node (leaf1) [stdnode, label={[tdlabel, xshift=2em,yshift=+1em]above left:$\tab{t_1}$}]{\input{graph0/tables/leaf0}};
\node (leaf1b) [stdnodenum,left=of leaf1,xshift=0.75em,yshift=0pt]{\input{graph0/tables/leaf0num}};
\node (leaf2b) [stdnodenum,right=1em of leaf1,xshift=-0.75em]  {\input{graph0/tables/leaf1num}};
\node (leaf2) [stdnode,right=-0.4em of leaf2b, label={[tdlabel, xshift=2em,yshift=+0.5em]above left:$\tab{t_2}$}]  {\input{graph0/tables/leaf1}};
\coordinate (middle) at ($ (leaf1.north east)!.5!(leaf2.north west) $);
\node (join) [stdnode,above=2mm of middle, label={[tdlabel, xshift=2em,yshift=+0.5em]above left:$\tab{t_3}$}] {\input{graph0/tables/join}};
\node (joinb) [stdnodenum,left=-0.4em of join] {\input{graph0/tables/joinnum}};

\draw (join) to (leaf1);
\draw (join) to (leaf2);
\end{tikzpicture}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "dbai-tr-2016-101"
%%% End:


==> graph0/tables/tables_asp.tex <==
\begin{tikzpicture}[node distance=1mm]
%\tikzset{every node/.style=tdnode}
\tikzset{every path/.style=thick}

\node (leaf1) [stdnode,label={[tdlabel,  xshift=1.25em,yshift=0.25em]above left:$\tab{t_1}$}] {\input{graph0/tables/leaf0_asp}};
\node (leaf1b) [stdnodenum,left=of leaf1,xshift=0.75em] {\input{graph0/tables/leaf0_aspnum}};
\node (leaf1c) [stdnodenum,right=of leaf1,xshift=-0.75em] {\input{graph0/tables/leaf0_aspnumb}};
\node (leaf2b) [stdnodenum,right=of leaf1c,xshift=-0.25em]  {\input{graph0/tables/leaf1_aspnum}};
\node (leaf2) [stdnode,right=of leaf2b, xshift=-0.75em, yshift=-0.4em, label={[tdlabel,  xshift=+0.1cm,yshift=0.25em]above:$\tab{t_2}$}]  {\input{graph0/tables/leaf1_asp}};
\node (leaf2c) [stdnodenum,right=of leaf2, xshift=-0.75em]  {\input{graph0/tables/leaf1_aspnumb}};
\coordinate (middle) at ($ (leaf1.north east)!.5!(leaf2.north west) $);
\node (join) [stdnode,above=2mm of middle, label={[tdlabel,  yshift=0.25em]above:$\tab{t_3}$}] {\input{graph0/tables/join_asp}};
\node (joinb) [stdnodenum,left=of join,xshift=0.75em] {\input{graph0/tables/join_aspnum}};
\node (joinc) [stdnodenum,right=of join,xshift=-0.75em] {\input{graph0/tables/join_aspnumb}};

\draw (join) to (leaf1);
\draw (join) to (leaf2);
\end{tikzpicture}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "dbai-tr-2016-101"
%%% End:


==> graph0/tables_inc/join_asp.tex <==
\begin{tabular}{c|c||c|c}
\multirow{2}{*}{$i$} & \multicolumn{1}{c}{$M_i$} & \multirow{2}{*}{$j$} & \multicolumn{1}{c}{$C_{j}$}\\
& $a$ && $a$\\\hline
%$1$ & & & \\\hline
%\multirow{1}{*}{$2$} & & \multirow{1}{*}{} & $1$ & &\\\hline
$3.1$ & \\\hline
$3.2\text{a}$ & T \\\hline
$3.2\text{b}$ & T & $3.2\text{b}.1$ & T \\
\end{tabular}


==> graph0/tables_inc/leaf0_asp.tex <==
\begin{tabular}{c|c|cc||c|c|cc}
\multirow{2}{*}{$i$} & \multicolumn{1}{c}{$M_i$} & \multicolumn{2}{c}{$\sigma_i$} & \multirow{2}{*}{$j$} & \multicolumn{1}{c}{$C_{j}$} & \multicolumn{2}{c}{$\rho_j$}\\
& $a$ & $r_1$ & $r_2$ && $a$ & $r_1$ & $r_2$ \\
\hline
%$2.1$ & & $+\infty$ & $0$\\\hline
$2.1\text{a}$ & T & $+\infty$ & $+\infty$ \\\hline %& $2.1.1$ & & $+\infty$ & $0$\\\hline
$2.1\text{b}$ & T & $+\infty$ & $+\infty$ & $2.1\text{b}.1$ & T & $+\infty$ & $+\infty$  \\\hline %& $2.1.1$ & & $+\infty$ & $0$\\\hline
$2.2$ & & $+\infty$ & $+\infty$ %\\\hline %& $2.1.1$ & & $+\infty$ & $0$\\\hline
%$2.3$ & T & $0$ & $+\infty$\\\hline %& $2.1.1$ & & $+\infty$ & $0$\\\hline
%$2.3$ & & $+\infty$ & $1$ & $2.3.1$ & & $+\infty$ & $0$\\\hline
%\multirow{2}{*}{$2.4$} & \multirow{2}{*}{T} & \multirow{2}{*}{$+\infty$} & \multirow{2}{*}{$1$} & $2.4.1$ & & $+\infty$ & $0$\\
%&&&& $2.4.2$ & & $+\infty$ & $1$\\\hline

%$1.1$ & & & T\\\hline
%$1.2$ & T & &\\\hline
%$1.3$ & T & & T & $1.3.1$ & T&\\\hline
%$1.4$ & & T & T\\\hline
%$1.5$ & T & T & T & $1.5.1$ & T&\\
\end{tabular}


==> graph0/tables_inc/leaf1_asp.tex <==
\begin{tabular}{c|cc|c||c|cc|c}
\multirow{2}{*}{$i$} & \multicolumn{2}{c}{$M_i$} & $\sigma_i$ & \multirow{2}{*}{$j$} & \multicolumn{2}{c}{$C_{j}$} & $\rho_j$\\
& $a$ & $d$ & $r_3$ && $a$ & $d$ & $r_3$ \\
\hline
%$3.1$ & && $0$\\\hline
$3.1$ & T & & $ +\infty$\\\hline %& $3.1.1$ & && $0$\\\hline
$3.2$ && T & $ +\infty$\\\hline %& $3.2.1$ & && $0$\\\hline
%\multirow{3}{*}{$3.4$} & \multirow{3}{*}{T} & \multirow{3}{*}{T} & \multirow{3}{*}{$+\infty$} & $3.4.1$ & && $0$\\
\multirow{2}{*}{$3.3$} & \multirow{2}{*}{T} & \multirow{2}{*}{T} & \multirow{2}{*}{$+\infty$} & $3.3.1$ & T && $+\infty$\\
%&&&& $3.4.2$ & T & & $+\infty$\\
&&&& $3.3.2$ && T & $+\infty$ %\\
%$2.2$ & & T\\\hline
%\multirow{2}{*}{$2.3$} & \multirow{2}{*}{T} & \multirow{2}{*}{T} & $2.3.1$ & T\\
%&&& $2.3.2$ & & T\\
\end{tabular}


==> graph0/tables_inc/leaf2_asp.tex <==
\begin{tabular}{c|cc|cc||c|cc|cc}
\multirow{2}{*}{$i$} & \multicolumn{2}{c}{$M_i$} & \multicolumn{2}{c}{$\sigma_i$} & \multirow{2}{*}{$j$} &  \multicolumn{2}{c}{$C_{j}$} & \multicolumn{2}{c}{$\rho_j$}\\
& $b$ & $c$ & $r_1$ & $r_2$ && $b$ & $c$ & $r_1$ & $r_2$ \\
\hline
$1.1$ & & & $+\infty$ & $0$\\\hline
$1.2$ & T & & $+\infty$ & $0$ & $1.2.1$ && & $+\infty$ & $0$\\\hline
$1.3$ & & T & $0$ & $+\infty$ & $1.3.1$ && & $+\infty$ & $0$\\\hline
\multirow{3}{*}{$1.4$} & \multirow{3}{*}{T} & \multirow{3}{*}{T} & \multirow{3}{*}{$0$} & \multirow{3}{*}{$+\infty$} & $1.4.1$ && & $+\infty$ & $0$\\
&&&&& $1.4.2$ &T && $+\infty$ & $0$ \\
&&&&& $1.4.3$ &&T & $0$ & $+\infty$ %\\%\hline

%$1.2$ & T & &\\\hline
%$1.3$ & T & & T & $1.3.1$ & T&\\\hline
%$1.4$ & & T & T\\\hline
%$1.5$ & T & T & T & $1.5.1$ & T&\\
\end{tabular}


==> graph0/tables_inc/tables_asp.tex <==
\begin{tikzpicture}[node distance=1mm]
%\tikzset{every node/.style=tdnode}
\tikzset{every path/.style=thick}

\node (leaf0) [stdnode,label={[tdlabel,  xshift=-0.1cm]left:$\tab{t_1}$}]{\input{graph0/tables_inc/leaf2_asp}};
\node (leaf1) [stdnode,above  = 0.1cm of leaf0,label={[tdlabel,  xshift=-0.1cm]left:$\tab{t_2}$}]{\input{graph0/tables_inc/leaf0_asp}};
\node (leaf2) [stdnode,right  = 0.1cm of leaf0, label={[tdlabel,  xshift=+0.1cm]right:$\tab{t_3}$}]  {\input{graph0/tables_inc/leaf1_asp}};
\coordinate (middle) at ($ (leaf1.north east)!.5!(leaf2.north west) $);
\node (join) [stdnode,above=1mm of leaf2, label={[tdlabel,  xshift=-0.0cm]right:$\tab{t_4}$}] {\input{graph0/tables_inc/join_asp}};

\draw (leaf0) to (leaf1);
\draw (join) to (leaf1);
\draw (join) to (leaf2);
\end{tikzpicture}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "dbai-tr-2016-101"
%%% End:


==> graph0_norm/tables/join.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$\langle \tuplecolor{\inputPredColor}{M_{11.i}} \rangle$}\\
\hline\hline
%$1$ & & & \\\hline
%\multirow{1}{*}{$2$} & & \multirow{1}{*}{} & $1$ & &\\\hline
$\langle \tuplecolor{\inputPredColor}{\emptyset} \rangle$ \\\hline
$\langle \tuplecolor{\inputPredColor}{\{a\}} \rangle$\\
\end{tabular}


==> graph0_norm/tables/join_asp.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$\langle \tuplecolor{\inputPredColor}{M_{11.i}}, \tuplecolor{\outputPredColor}{{\cal C}_{11.i}} \rangle$}\\
\hline\hline
%$1$ & & & \\\hline
%\multirow{1}{*}{$2$} & & \multirow{1}{*}{} & $1$ & &\\\hline
$\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\outputPredColor}{\emptyset} \rangle$\\\hline
$\langle \tuplecolor{\inputPredColor}{\{a\}}, \tuplecolor{\outputPredColor}{\emptyset} \rangle $\\\hline
$\langle \tuplecolor{\inputPredColor}{\{a\}}, \tuplecolor{\outputPredColor}{\{\{a\}\}} \rangle $\\
\end{tabular}


==> graph0_norm/tables/join_aspnum.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$i$}\\
\hline\hline
%$1$ & & & \\\hline
%\multirow{1}{*}{$2$} & & \multirow{1}{*}{} & $1$ & &\\\hline
$1$\\\hline
$2$\\\hline
$3$\\
\end{tabular}


==> graph0_norm/tables/join_aspnumb.tex <==
\begin{tabular}{c}
\multirow{1}{*}{$j$}\\
\hline\hline
%$1$ & & & \\\hline
%\multirow{1}{*}{$2$} & & \multirow{1}{*}{} & $1$ & &\\\hline
\\\hline
\\\hline
$1$\\
\end{tabular}


==> graph0_norm/tables/joinnum.tex <==
\begin{tabular}{c}
\multirow{1}{*}{$i$}\\
\hline\hline
%$1$ & & & \\\hline
%\multirow{1}{*}{$2$} & & \multirow{1}{*}{} & $1$ & &\\\hline
$1$ \\\hline
$2$\\
\end{tabular}


==> graph0_norm/tables/leaf0.tex <==
\begin{tabular}{l}
\multicolumn{1}{l}{$\langle \tuplecolor{\inputPredColor}{M_{4.i}} \rangle$}\\
%& $a$ & $b$ & $c$\\
\hline\hline
$\langle \tuplecolor{\inputPredColor}{\{c\}}\rangle$\\\hline
$\langle \tuplecolor{\inputPredColor}{\{a\}}\rangle$\\\hline
$\langle\tuplecolor{\inputPredColor}{\{a,c\}}\rangle$\\\hline
$\langle\tuplecolor{\inputPredColor}{\{b,c\}}\rangle$\\\hline
$\langle\tuplecolor{\inputPredColor}{\{a,b,c\}}\rangle$\\
\end{tabular}


==> graph0_norm/tables/leaf00.tex <==
\begin{tabular}{l}
\multicolumn{1}{l}{$\langle \tuplecolor{\inputPredColor}{M_{1.i}} \rangle$}\\
%& $a$ & $b$ & $c$\\
\hline\hline
$\langle \tuplecolor{\inputPredColor}{\emptyset}\rangle$
\end{tabular}


==> graph0_norm/tables/leaf00_asp.tex <==
\begin{tabular}{l}
\multicolumn{1}{l}{$\langle \tuplecolor{\inputPredColor}{M_{1.i}}, \tuplecolor{\outputPredColor}{{\cal C}_{1.i}}  \rangle$}\\
%& $a$ & $b$ & $c$\\
\hline\hline
$\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\outputPredColor}{\emptyset}\rangle$
\end{tabular}


==> graph0_norm/tables/leaf00_aspnum.tex <==
\begin{tabular}{c}
\multirow{1}{*}{$i$}\\ % & \multicolumn{1}{c}{$M_i$}\\
%& $a$ & $b$ & $c$\\
\hline\hline
$1$
\end{tabular}


==> graph0_norm/tables/leaf00_aspnumb.tex <==
\begin{tabular}{c}
\multirow{1}{*}{$j$}\\ % & \multicolumn{1}{c}{$M_i$}\\
%& $a$ & $b$ & $c$\\
\hline\hline
$1$
\end{tabular}


==> graph0_norm/tables/leaf00num.tex <==
\begin{tabular}{c}
\multirow{1}{*}{$i$}\\ % & \multicolumn{1}{c}{$M_i$}\\
%& $a$ & $b$ & $c$\\
\hline\hline
$1$
\end{tabular}


==> graph0_norm/tables/leaf0_asp.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$\langle \tuplecolor{\inputPredColor}{M_{4.i}}, \tuplecolor{\outputPredColor}{{\cal C}_{4.i}} \rangle $}\\
\hline\hline
$\langle \tuplecolor{\inputPredColor}{\{c\}}, \tuplecolor{\outputPredColor}{\emptyset} \rangle $\\\hline
%$1.1$ & & & T\\\hline
$\langle \tuplecolor{\inputPredColor}{\{a\}}, \tuplecolor{\outputPredColor}{\emptyset} \rangle $\\\hline
%$1.2$ & T & &\\\hline
$\langle \tuplecolor{\inputPredColor}{\{a,c\}}, \tuplecolor{\outputPredColor}{\{\{a\}\}} \rangle $\\\hline
%$1.3$ & T & & T & $1.3.1$ & T&\\\hline
$\langle \tuplecolor{\inputPredColor}{\{b,c\}}, \tuplecolor{\outputPredColor}{\emptyset} \rangle $\\\hline
$\langle \tuplecolor{\inputPredColor}{\{a,b,c\}}, \tuplecolor{\outputPredColor}{\{\{a\}\}} \rangle $\\
%$1.4$ & & T & T\\\hline
%$1.5$ & T & T & T & $1.5.1$ & T&\\
\end{tabular}


==> graph0_norm/tables/leaf0_aspnum.tex <==
\begin{tabular}{c}
\multirow{1}{*}{$i$}\\
\hline\hline
$1$\\\hline
$2$\\\hline
$3$\\\hline
$4$\\\hline
$5$
\end{tabular}



==> graph0_norm/tables/leaf0_aspnumb.tex <==
\begin{tabular}{c}
\multirow{1}{*}{$j$}\\
\hline\hline
\\\hline
\\\hline
$1$\\\hline
\\\hline
$1$\\
\end{tabular}


==> graph0_norm/tables/leaf0num.tex <==
\begin{tabular}{c}
\multirow{1}{*}{$i$}\\ % & \multicolumn{1}{c}{$M_i$}\\
%& $a$ & $b$ & $c$\\
\hline\hline
$1$ \\\hline
$2$ \\\hline
$3$ \\\hline
$4$ \\\hline
$5$ \\
\end{tabular}


==> graph0_norm/tables/leaf1.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$\langle \tuplecolor{\inputPredColor}{M_{9.i}} \rangle$}\\ % & \multicolumn{2}{c}{$M_i$}\\
%& $a$ & $d$ \\
\hline\hline
$\langle \tuplecolor{\inputPredColor}{\{a\}}\rangle$\\\hline
$\langle \tuplecolor{\inputPredColor}{\{d\}}\rangle$\\\hline
$\langle \tuplecolor{\inputPredColor}{\{a,d\}}\rangle$\\
\end{tabular}


==> graph0_norm/tables/leaf1_asp.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$\langle \tuplecolor{\inputPredColor}{M_{9.i}}, \tuplecolor{\outputPredColor}{{\cal C}_{9.i}} \rangle $}\\
\hline\hline
$\langle \tuplecolor{\inputPredColor}{\{ a\}}, \tuplecolor{\outputPredColor}{\emptyset} \rangle$\\\hline
$\langle \tuplecolor{\inputPredColor}{\{d\}}, \tuplecolor{\outputPredColor}{\emptyset} \rangle $\\\hline
$\langle \tuplecolor{\inputPredColor}{\{a,d\}}, \tuplecolor{\outputPredColor}{\{\{a\},} $\\
$\qquad\qquad \tuplecolor{\outputPredColor}{\{d\}\}}\rangle$\\
\end{tabular}


==> graph0_norm/tables/leaf1_aspnum.tex <==
\begin{tabular}{c}
\multirow{1}{*}{$i$}\\
\hline\hline
$1$\\\hline
$2$\\\hline
\multirow{2}{*}{$3$}\\
\end{tabular}


==> graph0_norm/tables/leaf1_aspnumb.tex <==
\begin{tabular}{c}
\multirow{1}{*}{$j$}\\
\hline\hline
\\\hline
\\\hline
$1$\\
$2$\\
\end{tabular}


==> graph0_norm/tables/leaf1num.tex <==
\begin{tabular}{c}
\multirow{1}{*}{$i$}\\ % & \multicolumn{2}{c}{$M_i$}\\
%& $a$ & $d$ \\
\hline\hline
$1$\\\hline
$2$\\\hline
$3$\\
\end{tabular}


==> graph0_norm/tables_inc/join.tex <==
\begin{tabular}{l}
\multirow{1}{*}{\pcrop$\langle \tuplecolor{\inputPredColor}{M_{6.i}}, \tuplecolor{\statePredColor}{\sigma_{6.i}} \rangle\quad\;\;\tab{6}\pcrop$}\\
\hline\hline
%$1$ & & & \\\hline
%\multirow{1}{*}{$2$} & & \multirow{1}{*}{} & $1$ & &\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{c\}}, \tuplecolor{\statePredColor}{\{r_1\mapstos0,r_2\mapstos\infty\}} \rangle\pcrop$ \\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_1\mapstos\infty,r_2\mapstos0\}} \rangle$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_1\mapstos\infty,r_2\mapstos1\}} \rangle$\\
\end{tabular}


==> graph0_norm/tables_inc/join_asp.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$\pcrop\langle \tuplecolor{\inputPredColor}{M_{6.i}}, \tuplecolor{\statePredColor}{\sigma_{6.i}}, \tuplecolor{\outputPredColor}{{\cal C}_{6.i}} \rangle\quad\;\tab{6}\pcrop$}\\
\hline\hline
%$1$ & & & \\\hline
%\multirow{1}{*}{$2$} & & \multirow{1}{*}{} & $1$ & &\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{c\}}, \tuplecolor{\statePredColor}{\{r_1\mapstos0,r_2\mapstos\infty\}}, \tuplecolor{\outputPredColor}{\{}$\\
$\quad\tuplecolor{\outputPredColor}{(\emptyset, \{r_1\mapstos\infty, r_2\mapstos0\})\}} \rangle\pcrop$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{c\}}, \tuplecolor{\statePredColor}{\{r_1\mapstos0,r_2\mapstos\infty\}}, \tuplecolor{\outputPredColor}{\{}$\\
$\quad\tuplecolor{\outputPredColor}{(\{c\}, \{r_1\mapstos1, r_2\mapstos\infty\}),}\pcrop$\\
$\quad\tuplecolor{\outputPredColor}{(\emptyset, \{r_1\mapstos\infty, r_2\mapstos0\}),}$\\
$\quad\tuplecolor{\outputPredColor}{(\emptyset, \{r_1\mapstos\infty, r_2\mapstos1\})\}}\rangle\pcrop$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_1\mapstos\infty,r_2\mapstos0\}}, \tuplecolor{\outputPredColor}{\emptyset} \rangle$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_1\mapstos\infty,r_2\mapstos1\}}, \tuplecolor{\outputPredColor}{\{}$\\
$\quad\tuplecolor{\outputPredColor}{(\emptyset, \{r_1\mapstos\infty, r_2\mapstos0\})\}} \rangle\pcrop$%\\\hline
\end{tabular}


==> graph0_norm/tables_inc/leaf0.tex <==
\begin{tabular}{l}
\multicolumn{1}{l}{$\pcrop\langle \tuplecolor{\inputPredColor}{M_{4.i}}, \tuplecolor{\statePredColor}{\sigma_{4.i}} \rangle \quad\;\;\tab{4}\pcrop$}\\
%& $a$ & $b$ & $c$\\
\hline\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{c\}}, \tuplecolor{\statePredColor}{\{r_1\mapstos 0,r_2\mapstos\infty\}} \rangle\pcrop$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_1\mapstos\infty,r_2\mapstos0\}}\rangle$\\
\end{tabular}


==> graph0_norm/tables_inc/leaf00.tex <==
\begin{tabular}{l}
\multicolumn{1}{l}{$\pcrop\langle \tuplecolor{\inputPredColor}{M_{1.i}}, \tuplecolor{\statePredColor}{\sigma_{1.i}} \rangle\;\;\tab{1}\pcrop$}\\
%& $a$ & $b$ & $c$\\
\hline\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\emptyfunc}\rangle$
\end{tabular}


==> graph0_norm/tables_inc/leaf00_asp.tex <==
\begin{tabular}{l}
\multicolumn{1}{l}{$\pcrop\langle \tuplecolor{\inputPredColor}{M_{1.i}}, \tuplecolor{\statePredColor}{\sigma_{1.i}}, \tuplecolor{\outputPredColor}{{\cal C}_{1.i}}  \rangle\;\;\tab{1}\pcrop$}\\
%& $a$ & $b$ & $c$\\
\hline\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\emptyfunc}, \tuplecolor{\outputPredColor}{\emptyset}\rangle$
\end{tabular}


==> graph0_norm/tables_inc/leaf0_asp.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$\pcrop\langle \tuplecolor{\inputPredColor}{M_{4.i}}, \tuplecolor{\statePredColor}{\sigma_{4.i}}, \tuplecolor{\outputPredColor}{{\cal C}_{4.i}} \rangle\quad\tab{4}\pcrop$}\\
\hline\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{c\}}, \tuplecolor{\statePredColor}{\{r_1\mapstos0,r_2\mapstos\infty\}}, \tuplecolor{\outputPredColor}{\{}$\\
$\quad\tuplecolor{\outputPredColor}{(\emptyset, \{r_1\mapstos\infty, r_2\mapstos0\})\}}\rangle\pcrop$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_1\mapstos\infty,r_2\mapstos0\}}, \tuplecolor{\outputPredColor}{\emptyset} \rangle$
\end{tabular}


==> graph0_norm/tables_inc/leaf1.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$\pcrop\langle \tuplecolor{\inputPredColor}{M_{15.i}}, \tuplecolor{\statePredColor}{\sigma_{15.i}} \rangle\pcrop$}\\ % & \multicolumn{2}{c}{$M_i$}\\
%& $a$ & $d$ \\
\hline\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a\}}, \tuplecolor{\statePredColor}{\emptyfunc}\rangle$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{d\}}, \tuplecolor{\statePredColor}{\emptyfunc}\rangle$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a,d\}}, \tuplecolor{\statePredColor}{\emptyfunc}\rangle$\\
\end{tabular}


==> graph0_norm/tables_inc/leaf1_asp.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$\pcrop\langle \tuplecolor{\inputPredColor}{M_{15.i}}, \tuplecolor{\statePredColor}{\sigma_{15.i}}, \tuplecolor{\outputPredColor}{{\cal C}_{15.i}} \rangle\;\;\tab{15}\pcrop$}\\
\hline\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a\}},  \tuplecolor{\statePredColor}{\emptyfunc}, \tuplecolor{\outputPredColor}{\emptyset} \rangle$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{d\}}, \tuplecolor{\statePredColor}{\emptyfunc}, \tuplecolor{\outputPredColor}{\emptyset} \rangle $\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a,d\}}, \tuplecolor{\statePredColor}{\emptyfunc}, \tuplecolor{\outputPredColor}{\{}$%\\
$\tuplecolor{\outputPredColor}{(\{a\}, \emptyfunc),}\pcrop$\\
$\quad\tuplecolor{\outputPredColor}{(\{d\}, \emptyfunc)\}}\rangle$
\end{tabular}


==> graph0_norm/tables_inc/r14.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$\pcrop\langle \tuplecolor{\inputPredColor}{M_{9.i}}, \tuplecolor{\statePredColor}{\sigma_{9.i}} \rangle$}\\
\hline\hline
%$1$ & & & \\\hline
%\multirow{1}{*}{$2$} & & \multirow{1}{*}{} & $1$ & &\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a\}}, \tuplecolor{\statePredColor}{\{r_1\mapstos\infty\}} \rangle\pcrop$\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_1\mapstos\infty\}} \rangle$\\%\hline
%$\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_1\mapstos\infty,r_2\mapstos1\}} \rangle$\\
\end{tabular}


==> graph0_norm/tables_inc/r14_asp.tex <==
\begin{tabular}{l}
\multirow{1}{*}{$\pcrop\langle \tuplecolor{\inputPredColor}{M_{9.i}}, \tuplecolor{\statePredColor}{\sigma_{9.i}}, \tuplecolor{\outputPredColor}{{\cal C}_{9.i}} \rangle\,\;\;\qquad\tab{9}\pcrop$}\\
\hline\hline
%$1$ & & & \\\hline
%\multirow{1}{*}{$2$} & & \multirow{1}{*}{} & $1$ & &\\\hline
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a\}}, \tuplecolor{\statePredColor}{\{r_1\mapstos\infty\}}, \tuplecolor{\outputPredColor}{\emptyset}\rangle$\\\hline
%
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a\}}, \tuplecolor{\statePredColor}{\{r_1\mapstos\infty\}}, \tuplecolor{\outputPredColor}{\{}$%\\
$\tuplecolor{\outputPredColor}{(\emptyset,\hspace{-0.2em}\{r_1\mapstos0\}),}\pcrop$\\
$\quad\tuplecolor{\outputPredColor}{(\{a\}, \{r_1\mapstos\infty\})\}}\rangle$\\\hline
%
$\pcrop\langle \tuplecolor{\inputPredColor}{\{a\}}, \tuplecolor{\statePredColor}{\{r_1\mapstos\infty\}}, \tuplecolor{\outputPredColor}{\{}$\\
$\quad\tuplecolor{\outputPredColor}{(\emptyset, \{r_1\mapstos0\}),}$%\\
$\tuplecolor{\outputPredColor}{(\emptyset, \{r_1\mapstos1\}),}\pcrop$\\
$\quad\tuplecolor{\outputPredColor}{(\{a\}, \{r_1\mapstos\infty\}),}$\\
$\quad\tuplecolor{\outputPredColor}{(\{a\}, \{r_1\mapstos1\})\}}\rangle$\\\hline
%
$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_1\mapstos\infty\}}, \tuplecolor{\outputPredColor}{\emptyset}\rangle$\\\hline
%
$\pcrop\langle \tuplecolor{\inputPredColor}{\emptyset}, \tuplecolor{\statePredColor}{\{r_1\mapstos\infty\}}, \tuplecolor{\outputPredColor}{\{}$%\\
$\tuplecolor{\outputPredColor}{(\emptyset, \{r_1\mapstos1\})\}}\rangle\pcrop$\\
\end{tabular}

